Fighting noise and imbalance in Action Unit detection problems

Action Unit (AU) detection aims at automatically caracterizing facial expressions with the muscular activations they involve. Its main interest is to provide a low-level face representation that can be used to assist higher level affective computing tasks learning. Yet, it is a challenging task. Indeed, the available databases display limited face variability and are imbalanced toward neutral expressions. Furthermore, as AU involve subtle face movements they are difficult to annotate so that some of the few provided datapoints may be mislabeled. In this work, we aim at exploiting label smoothing ability to mitigate noisy examples impact by reducing confidence [1]. However, applying label smoothing as it is may aggravate imbalance-based pre-existing under-confidence issue and degrade performance. To circumvent this issue, we propose Robin Hood Label Smoothing (RHLS). RHLS principle is to restrain label smoothing confidence reduction to the majority class. In that extent, it alleviates both the imbalance-based over-confidence issue and the negative impact of noisy majority class examples. From an experimental standpoint, we show that RHLS provides a free performance improvement in AU detection. In particular, by applying it on top of a modern multi-task baseline we get promising results on BP4D and outperform state-of-the-art methods on DISFA.

==> tables/bp4d/rebalancing_ls.tex <==
\resizebox{1.03\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\alpha_b & epoch & Valid Avg. & 4/5 Test Avg. & Mean (Std) Test Avg. & Max Test Avg. \\
\hline
0.0 & 61.0 & 61.9 & 62.0 (0.07) & 63.1 \\
0.25 & 60.9 & 61.8 & - & - \\
0.5 & 60.3 & 61.8 & - & - \\
0.75 & 60.9 & 61.9 & - & - \\
1.0 & 60.2 & 61.4 & - & - \\
\hline
\end{tabular}}

==> tables/bp4d/size.tex <==
\resizebox{1.03\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
size & epoch & Valid Avg. & 4/5 Test Avg. & Mean (Std) Test Avg. & Max Test Avg. \\
\hline
XXS & 59.5 & 60.4 & - & - \\
XS & 61.0 & 61.9 & - & - \\
S & 60.7 & 61.3 & - & - \\
M & 60.7 & 61.3 & - & - \\
\hline
\end{tabular}}

==> tables/bp4d/sota_comparaison.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\footnotesize {\bf{F1 Score-AU}} &1 & 2 & 4 & 6 & 7 & 10 & 12 & 14 & 15 & 17 & 23 & 24 & {\bf{Avg.}} \\
\hline
%\footnotesize DRML \cite{zhao2016deep} & 36.4 & 41.8 & 43.0 & 55.0 & 67.0 & 66.3 & 65.8 & 54.1 & 33.2 & 48.0 & 31.7 & 30.0 & 48.3 \\
%\footnotesize EAC-NET \cite{li2018eac} & 39.0 & 35.2 & 48.6 & 76.1 & 72.9 & 81.9 & 86.2 & 58.8 & 37.5 & 59.1 & 35.9 & 35.8 & 55.9 \\
%\footnotesize DSIN \cite{corneanu2018deep} & 51.7 & 40.4 & 56.6 & 76.1 & 73.5 & 79.9 & 85.4 & 62.7 & 37.3 & 62.9 & 38.8 & 41.6 & 58.9 \\
\footnotesize JAANet \cite{shao2018deep} & 47.2 & 44.0 & 54.9 & 77.5 & 74.6 & 84.0 & 86.9 & 61.9 & 43.6 & 60.3 & 42.7 & 41.9 & 60.0 \\
%\footnotesize LP-Net \cite{niu2019local} & 43.4 & 38.0 & 54.2 & 77.1 & 76.7 & 83.8 & 87.2 & 63.3 & 45.3 & 60.5 & 48.1 & 54.2 & 61.0 \\
%\footnotesize CMS \cite{sankaran2019representation} & 49.1 & 44.1 & 50.3 & 79.2 & 74.7 & 80.9 & 88.3 & 63.9 & 44.4 & 60.3 & 41.4 & 51.2 & 60.6 \\
\footnotesize ARL \cite{shao2019facial} & 45.8 & 39.8 & 55.1 & 75.7 & 77.2 & 82.3 & 86.6 & 58.8 & 47.6 & 62.1 & 47.7& 55.4 & 61.1 \\
%\footnotesize SRERL \cite{li2019semantic} & 46.9 & 45.3 & 55.6 & 77.1 & 78.4 & 83.5 & 87.6 & 63.9 & 52.2 & \best{63.9} & 47.1 & 53.3 & 62.1 \\
\footnotesize JÂANET \cite{shao2020jaa} & 53.8 & 47.8 & 58.2 & \best{78.5} & 75.8 & 82.7 & \best{88.2} & 63.7 & 43.3 & 61.8 & 45.6 & 49.9 & 62.4 \\
\footnotesize UGN-B \cite{song2021uncertain} & 54.2 & 46.4 & 56.8 & 76.2 & 76.7 & 82.4 & 86.1 & 64.7 & 51.2 & 63.1 & 48.5 & 53.6 & 63.3 \\
%\footnotesize HMP-PS \cite{song2021hybrid} & 53.1 & 46.1 & 56.0 & 76.5 & 76.9 & 82.1 & 86.4 & 64.8 & 51.5 & 63.0 & 49.9 & 54.5 & 63.4 \\
%\footnotesize SEV-Net \cite{yang2021exploiting} &  58.2 & \best{50.4} & 58.3 & \best{81.9} & 73.9 & 87.8 & 87.5 & 61.6 & 52.6 & 62.2 & 44.6 & 47.6 & 63.9 \\
\footnotesize FAUwT \cite{jacob2021facial} & 51.7 & \best{49.3} & 61.0 & 77.8 & \best{79.5} & 82.9 & 86.3 & \best{67.6} & 51.9 & 63.0 & 43.7 & \best{56.3} & 64.2 \\
\footnotesize MONET  \cite{tallec2022multi} & \best{54.5} & 45.0 & \best{61.5} & 75.9 & 78.0 & \best{84.5} & 87.6 & 65.1 & \best{54.8} & 60.5 & \best{53.0} & 53.2 & \best{64.5} \\
\hline
\footnotesize Baseline & 52.2 & 41.5 & 59.5 & 77.7 & 76.7 & 83.1 & \best{88.2} & 56.7 & 48.8 & 62.3 & 47.6 & 49.0 & 61.9 \\
\footnotesize RHLS  & 53.2 & 44.9 & 58.6 & \best{78.5} & 77.5 & 83.1 & 88.1 & 61.3 & 50.7 & 62.6 & 47.0 & 49.6 & 63.0 \\
\hline 
\end{tabular}}

==> tables/disfa/rebalancing_ls.tex <==
\resizebox{1.03\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\alpha_b & epoch & Valid Avg. & 4/5 Test Avg. & Mean (Std) Test Avg. & Max Test Avg. \\
\hline
0.0 & 61.0 & 61.9 & 62.0 (0.07) & 63.1 \\
0.25 & 60.9 & 61.8 & - & - \\
0.5 & 60.3 & 61.8 & - & - \\
0.75 & 60.9 & 61.9 & - & - \\
1.0 & 60.2 & 61.4 & - & - \\
\hline
\end{tabular}}

==> tables/disfa/rebalancing_ls_valid.tex <==
%\resizebox{1.03\linewidth}{!}{
%\begin{tabular}{|c|c|}
%\hline
%$\beta$ & Mean Valid F1Score \\%& Mean Eval F1Score  \\
%\hline
%0.0 & 55.7 \\ % & 63.0 \\
%0.25 & \bf{57.7} \\ % & \bf{65.8} \\
%0.5 & 56.4 \\ % & - \\
%0.75 & 56.5 \\ % & - \\
%1.0 & 47.4 \\ % & - \\
%\hline
%\end{tabular}}

\resizebox{1.03\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$\beta$ & 0 & 0.25 & 0.5 & 0.75 & 1.0 \\%& Mean Eval F1Score  \\
\hline
Valid Score & 55.7 & \bf{57.7} & 56.4 & 56.5 & 47.4 \\ % & 
\hline
\end{tabular}}

==> tables/disfa/size.tex <==
\resizebox{1.03\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
size & epoch & Valid Avg. & 4/5 Test Avg. & Mean (Std) Test Avg. & Max Test Avg. \\
\hline
XXS & 54.2 & 61.5 & 61.5 & - \\
XS & 52.2 & 62.5 & 61.9 & - \\
S & 53.1 & 61.2 & 63.0 & - \\
M & 55.0 & 59.8 & - & - \\
\hline
\end{tabular}}

==> tables/disfa/sota_comparaison.tex <==
\resizebox{0.78\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\footnotesize \bf{F1 Score-AU} &1 &2 & 4 & 6 & 9 & 12 & 25 & 26 & \textbf{Avg.} \\
\hline
%\footnotesize DRML \cite{zhao2016deep} & 17.3 & 17.7 & 37.4 & 29.0 & 10.7 & 37.7 & 38.5 & 20.1 & 26.7 \\
%\footnotesize EAC-NET \cite{li2018eac} & 41.5 & 26.4 & 66.4 & 50.7 & 8.5 & \best{89.3} & 88.9 & 15.6 & 48.5 \\
%\footnotesize DSIN \cite{corneanu2018deep} & 42.4 & 39.0 & 68.4 & 28.6 & 46.8 & 70.8 & 90.4 & 42.2 & 53.6 \\
%\footnotesize SRERL \cite{li2019semantic} & 45.7 & 47.8 & 59.6 & 47.1 & 45.6 & 73.5 & 84.3 & 43.6 & 55.9 \\
\footnotesize JAANet \cite{shao2018deep} & 43.7 & 46.2 & 56.0 & 41.4 & 44.7 & 69.6 & 88.3 & 58.4 & 56.0 \\
%\footnotesize LP-Net \cite{niu2019local} & 29.9 & 24.7 & \sebest{72.7} & 46.8 & 49.6 & 72.9 & 93.8 & 65.0 & 56.9 \\
%\footnotesize CMS \cite{sankaran2019representation} & 40.2 & 44.3 & 53.2 & \best{57.1} & 50.3 & 73.5 & 81.1 & 59.7 & 57.4 \\
\footnotesize ARL \cite{shao2019facial} & 43.9 & 42.1 & 63.6 & 41.8 & 40.0 & \best{76.2} & 95.2 & 66.8 & 58.7 \\
%\footnotesize SEV-Net \cite{yang2021exploiting} & 55.3 & 53.1 & 61.5 & 53.6 & 38.2 & 71.6 & \best{95.7} & 41.5 & 58.8 \\
\footnotesize UGN-B \cite{song2021uncertain} & 43.3 & 48.1 & 63.4 & 49.5 & 48.2 & 72.9 & 90.8 & 59.0 & 60.0 \\
%\footnotesize HMP-PS \cite{song2021hybrid} & 38.0 & 45.9 & 65.2 & 50.9 & \best{50.8} & 76.0 & 93.3 & \best{67.6} & 61.0 \\
\footnotesize FAUwT \cite{jacob2021facial} & 46.1 & 48.6 & \best{72.8} & 56.7 & 50.0 & 72.1 & 90.8 & 55.4 & 61.5 \\
\footnotesize JÂANET \cite{shao2020jaa} & 62.4 & 60.7 & 67.1 & 41.1 & 45.1 & 73.5 & 90.9 & 67.4 & 63.5 \\
\footnotesize MONET \cite{tallec2022multi} & 55.8 & 60.4 & 68.1 & 49.8 & 48.0 & 73.7 & 92.3 & 63.1 & 63.9 \\
\hline
\footnotesize Baseline (ours) & 63.3 & 57.9 & 66.4 & 43.9 & 41.5 & 75.8 & 94.0 & 61.8 & 63.1 \\
\footnotesize RHLS (ours)& \best{67.2} & \best{64.6} & 66.7 & 46.6 & 47.2 & 75.1 & 93.9 & 65.5 & \best{65.8} \\
\hline
\end{tabular}
 }
